Model-Adaptive Interface Generation for Data-Driven Discovery

Discovery of new knowledge is increasingly data-driven, predicated on a team's ability to collaboratively create, find, analyze, retrieve, and share pertinent datasets over the duration of an investigation. This is especially true in the domain of scientific discovery where generation, analysis, and interpretation of data are the fundamental mechanisms by which research teams collaborate to achieve their shared scientific goal. Data-driven discovery in general, and scientific discovery in particular, is distinguished by complex and diverse data models and formats that evolve over the lifetime of an investigation. While databases and related information systems have the potential to be valuable tools in the discovery process, developing effective interfaces for data-driven discovery remains a roadblock to the application of database technology as an essential tool in scientific investigations. In this paper, we present a model-adaptive approach to creating interaction environments for data-driven discovery of scientific data that automatically generates interactive user interfaces for editing, searching, and viewing scientific data based entirely on introspection of an extended relational data model. We have applied model-adaptive interface generation to many active scientific investigations spanning domains of proteomics, bioinformatics, neuroscience, occupational therapy, stem cells, genitourinary, craniofacial development, and others. We present the approach, its implementation, and its evaluation through analysis of its usage in diverse scientific settings.

==> parts/usecases-deadtext.tex <==
\subsection{Presentation Customization Use Cases}\label{sec:examples}

PERHAPS THIS SHOULD BE RETITLED TO BE: EXAMPLE OF AN ANNOTATION, OR SOMETHING LIKE THAT. NEED TO RECOVER TEXT THAT DESCRIBES THIS.  WE WHOULD PROBABLY PUT IN COMMENTS IN THE ANNOTATION?

 We describe how \chaise\ applications are customized in actual deployment examples. The examples are not meant to be exhaustive, but to illustrate common customization patterns observed within and across deployments. We use GUDMAP/RBK model and annotations for illustration. 

\subsubsection{Table-level annotations}
By default, \chaise\ displays all table columns in the order created in the database. However, many tables are often customized their displayed columns in different contexts using the visible-columns annotation ({\tt tag:isrd.isi.edu,2016:visible-columns}). Figure~\ref{fig:table-annotations} shows all the table-level annotations associated with the Study table. For brevity, we only include a few top columns in our annotation examples; the rest of visible columns (or visible foreign keys) are defined similarly. Figures ~\ref{fig:gudmap-study-recordedit}, ~\ref{fig:gudmap-study-recordset}, and~\ref{fig:gudmap-study-record} show the actual displays of the Study table consisting of both native and denormalized pseudo columns according to the visible-columns annotation. 
The RecordEdit app renders the {\em entry} context for the input form. The recordset app renders the {\em compact} context for the main result table, and {\em facet} context for the search facets on the left panel. The record app renders the {\em detailed} context for the table summary, and {\em compact} context for related tables.   

Columns can be directly defined in the visible-columns or predefined under the source-definitions annotation ({\tt tag:isrd.isi.edu,2019:source-definitions}) and later referenced using the {\em source\-key} attribute.
The {\em source} attribute specifies how a column should be retrieved. A string (e.g. "RID", "Title") indicates a native column name while a foreign key path indicates a pseudo-column (see "Experiment\_Type" source attribute under "source-definitions" tag, for an example). A foreign key path consists of one or more foreign key objects followed by an end column in the final table. An end key column (e.g. {\em RID}) indicates an entity mode implying the whole row should be retrieved, while the non-key column indicates that only the specified column values should be retrieved. A foreign key object is a key-value pair specifying its direction (i.e. "inbound" v.s. "outbound") and unique name (i.e. a two-element array of schema and foreign key names e.g. ["RNASeq", "Experiment\_Study\_fkey"]). For example, specified under the source-definitions annotation, the "Experiment\_Type" is referring to the "Experiment\_Type" column residing in the Experiment table, and the "Anatomical\_Source" is referring to the "Name" column of the Tissue table through the specified foreign key path connecting from the Study to the Tissue tables through the Experiment, Replicate, Specimen, and Specimen\_Tissue tables. The "aggregate" key-value indicates the aggregation function applied to the column values; {\em array\_d} for distinct elements, and {\em cnt\_d} for the number of distinct elements associated with the column.

In addition to column list, other presentations can also be tweaked. The {\em display} property allows custom composition and display through templating and markdown. For example, the "Summary" column in the search result table is a composition of many aggregated pseudo-columns displaying in a bullet list. The {\em markdown\_name} enables overriding of column names (e.g. "Specimen\_Anatomical\_Source" instead of "Specimen\_Tissue" is used for the facet name).

\subsubsection{Table display}
The table-display annotation ({\tt tag:isrd.isi.edu,2016:table-display}) is used to tweak table presentation such as row order, row name. By default, the shortest key is used for row sorting, and the row names are derived based on certain column names (e.g. title, name) or the shortest key. The Study table is customized to sort rows based on RMT (Record Modified Time) in the descending order (Figure~\ref{fig:gudmap-study-recordset}), and the name of a specific entity is a concatenation of RID, ":", and Title. Row names are displayed on individual Record page title (e.g. a study page title in Figure~\ref{fig:gudmap-study-record}), and where foreign key references are in all apps (e.g. "Curation\_Status") .  

\subsubsection{Visible related tables}
By default, the Record app displays all tables directly referenced by the table of interest (e.g. direct inbound tables) under the related table sections. The visible-foreign-keys annotation ({\tt tag:isrd.isi.edu,2016:visible-foreign-keys}) overrides this default. Similar to the visible-column annotation, indirectly related tables can be denormalized and included for display using the source syntax. The named sources under the source-definitions annotation can be referenced in the visible-foreign-keys annotation. Figure~\ref{fig:gudmap-study-record} shows a list of displayed related tables under the Sections left panel; these tables are not visible in the screenshot.    

\subsubsection{Integrated visualization}
A visualization associated with a column can be flexibly integrated in~\chaise\ using {\em column-display} annotation({\tt tag:isrd.isiedu,2016:column-display}). Figure~\ref{fig:column-annotations} shows the annotation associated with the Study {\em Cellbrowser\_URL} column containing a URL to the Cell Browser single cell data visualization application. \chaise\ extends its markdown module to support an {\em iframe} markdown tag (i.e. {\tt :::iframe [<caption>](<URL>){<properties>} \textbackslash n :::}) that allows a trusted URL to be incorporated into the page using the iframe. The extension also supports a linkable caption. On the Study Record page (Figure~\ref{fig:gudmap-study-record}), the Cell Browser is rendered in a 1000x600 iframe window with the caption that navigates directly to the full Cell Browser page.     
  
\subsubsection{Role-based column and row visibility}
Certain columns and rows are usually visible to different user roles. In GUDMAP/RBK, only entities that are released are visible to the public. To achieve this, a {\em Curation\_Status} column is included in all primary tables associated with different assay types, as exemplified by the Study table metadata. The {\em Curation\_Status} tracks the status of individual entities in the curation process e.g. {\em In preparation}, {\em PI review}, {\em Biocurator review}, or {\em Release} and is used to determine row-level access. Moreover, the Curation\_Status itself is hidden to the public. 

With this policy, when an anonymous user engages with \chaise, the returned role-based model (as shown in Figure~\ref{fig:approach}) will omit all the hidden columns, and the role-based data will only include the released entities. \chaise\ will apply its presentation tweaks only to the reachable columns in the annotations. Curation\_Status is not present in the model, therefore will not be displayed. Additionally, since anonymous users have read-only access, all the editing controls will be omitted.  


%\begin{figure}[]
%  \centering
%  % include first image
%  \frame{\includegraphics[width=\linewidth]{figures/annotation-all.pdf}}
%  \caption{Study related table and column annotations}
%  \label{fig:table-annotations}
%\end{figure}

\begin{figure}[ht]
\begin{subfigure}{\textwidth}
  \centering
  % include first image
  \frame{\includegraphics[width=\linewidth]{figures/annotation.pdf}}
  \caption{Table annotations}
  \label{fig:table-annotations}
\end{subfigure}
\begin{subfigure}{\textwidth}
  \centering
  % include second image
  \frame{\includegraphics[width=\linewidth]{figures/annotation-column.pdf}}
  \caption{Column annotations}
  \label{fig:column-annotations}
\end{subfigure}
\caption{GUDMAP/RBK Study related annotations}
\label{fig:annotation}
\end{figure}


